Grand Schnyder Woods

We define a far-reaching generalization of Schnyder woods which encompasses many classical combinatorial structures on planar graphs. Schnyder woods are defined for planar triangulations as certain triples of spanning trees covering the triangulation and crossing each other in an orderly fashion. They are of theoretical and practical importance, as they are central to the proof that the order dimension of any planar graph is at most 3, and they are also underlying an elegant drawing algorithm. In this article we extend the concept of Schnyder wood well beyond its original setting: for any integer d>2 we define a ``grand-Schnyder'' structure for (embedded) planar graphs which have faces of degree at most d and non-facial cycles of length at least d. We prove the existence of grand-Schnyder structures, provide a linear construction algorithm, describe 4 different incarnations (in terms of tuples of trees, corner labelings, weighted orientations, and marked orientations), and define a lattice for the set of grand Schnyder structures of a given planar graph. We show that the grand-Schnyder framework unifies and extends several classical constructions: Schnyder woods and Schnyder decompositions, regular edge-labelings (a.k.a. transversal structures), and Felsner woods.

==> necessity.tex <==
%\documentclass{amsart}
%\input{defs}
%\begin{document}
%\section{Necessity proofs}

\subsection{Necessity proof for Grand Schnyder structures}


Let $G$ be a $d$-map, and let $G^+$ be the angular map of $G$. A \emph{star cycle} of $G^+$ is a cycle made of star edges only. 

 \begin{lemma}\label{lem:star_cycle}
 Let $G$ be a $d$-map endowed with a $d$-GS angular orientation. Let $C'$ be a star cycle of $G^+$, and let $\ell$ be its enclosing length (as defined in Section~\ref{sec:lattice_GS}).  
 Then the inward degree of $C'$ is equal to $\ell-d$. 
\end{lemma}
\begin{proof}
The proof is exactly the same as the one of Lemma~\ref{lem:compa}. 
\end{proof}


\begin{figure}
\begin{center}
\includegraphics[width=13cm]{C0}
\end{center}
\caption{For $G$ a $d$-map, the fact that a non-facial cycle $C$ of $G$ is not the enclosing cycle of a star cycle of $G^+$ is witnessed by the existence of two edges $e_1,e_2$  on $C$ that are incident to a same original face $f$ inside $C$, of degree smaller than $d$, such that each of the two portions of $C$ separated by $\{e_1,e_2\}$ contains at least one edge not incident to $f$.
This produces two non-facial cycles of $G$ whose interior is included in the interior of $C$. 
}
\label{fig:C0}
\end{figure}

\begin{prop}\label{prop:necessity_GS}
If a $d$-map $G$ admits a $d$-GS angular orientation, then $G$ is $d$-adapted.
\end{prop}
\begin{proof}
The first step is to show that $G$ has to be non-separable, i.e., $G^+$ has no star-cycle of length $2$. Assume such a cycle $C'$ exists, and let $C$ be its
enclosing cycle. Letting $f$ be the inner face of $G$ corresponding to the star vertex $s$ on $C'$, clearly all edges on $C$ are on the contour of~$f$. By Lemma~\ref{lem:star_cycle}, $C$ has length at least $d$. Hence, $s$ is incident to at least $d-1$ star edges in the exterior of $C'$. Since $s$ is incident to two edges on $C'$, we conclude that $s$ has degree larger than $d$, in contradiction with the fact that $G$ is a $d$-map. Hence, $G$ is non-separable.

Let $X$ be the set of non-facial
cycles of $G$ of length smaller than $d$. Assume $X$ is not empty, and let $C_0$ be a minimal element of $X$ (i.e., there is no other $C_1\in X$ such that the interior of $C_1$ is included in the interior of $C_0$). 
Since $C_0$ has length smaller than $d$, by Lemma~\ref{lem:star_cycle} it can not be the enclosing cycle of a compatible cycle. This means that there exists a face $f$ of $G$ 
inside $C$ that shares at least one edge with $C$, but such that the edges along $f$ that are on $C$ do not form a contiguous set on the contour of $f$. Since $G$
is non-separable, this set of edges is neither contiguous on $C$. 
Hence, we are in the situation shown in  Figure~\ref{fig:C0}. 
We have $L_1+L_2+2=\mathrm{length}(C_0)<d$ and 
$\ell_1+\ell_2+2=\mathrm{deg}(f)\leq d$, so $(L_2+\ell_1+2)+(L_1+\ell_2+2)<2d$, thus at least one of the two cycles on the right-side of  Figure~\ref{fig:C0} has length strictly smaller than~$d$, yielding a contradiction to the minimality of~$C_0$.  
\end{proof}

\subsection{Necessity proof for weak Grand Schnyder structures}

A \emph{relaxed weighted orientation} is a weighted orientation where the arc-weights are in 
$\mathbb{Z}$. As usual, the outgoing weight of a vertex $v$ is the sum of the weights of the arcs going out of $v$, the weight of an edge is the sum of weights of its two arcs, and the inward degree of a cycle is the sum of the weights of the arcs inside the cycle and with their initial vertex on the cycle.  
For a $d$-map $G$, with $G^+$ the angular map, a \emph{relaxed $d$-GS angular orientation} of $G$ is a relaxed weighted orientation of $G^+$ with exactly the same requirements as in Definition~\ref{def:angular}, the only difference being that negative arc-weights are allowed. 

\begin{lemma}\label{lem:weak_compatible}
Let $G$ be a $d$-map. Let $C'$ be a star cycle of $G^+$, and let $\ell$ be its enclosing length. Then, in any relaxed $d$-GS angular orientation of $G$, the inward degree of $C'$ is equal to $\ell-d$. 
\end{lemma}
\begin{proof}
The proof of Lemma~\ref{lem:star_cycle} (i.e., the proof of Lemma~\ref{lem:compa}) can be copied verbatim (it does not use positivity of arc-weights). 
\end{proof}

For $G$ a $d$-map, we call \emph{special quadrangle} of $G^+$ a 4-cycle whose contour contains the two extremities of a 
special original edge $e$ (edge with $e_d=-1$) and the two star-vertices for the faces of $G$ incident to $e$. 



\begin{lemma}\label{lem:transition}
If a $d$-map $G$ admits a weak $d$-GS angular orientation, then $G$ admits a relaxed $d$-GS angular orientation (on $G^+$) such that any cycle of $G^+$ has nonnegative inward degree, except for the special quadrangles, which have inward degree~$-1$.  
\end{lemma}
\begin{proof}
By applying the rules of Figure~\ref{fig:local_rules_transition} at each edge-vertex of a weak $d$-GS angular orientation, we obtain a relaxed $d$-GS angular orientation, where the only arcs of negative weight are on the special original  edges: each such edge has an arc of weight $-1$ and an arc of weight $0$. Now let $C'$ be a cycle in $G^+$, and consider an arc of weight $-1$ having its origin on $C'$, on a special original edge $e$. Then one easily checks that, if none of the $4$ green edges arising from $e$ (in the intermediate step in Figure~\ref{fig:local_rules_transition}) contributes to the inward degree of $C'$ (i.e., has its origin on $C'$ and its end inside $C'$), then $C'$ is reduced to the special quadrangle enclosing $e$. Hence, only these cycles have negative inward degree (equal to $-1$), any other cycle has nonnegative inward degree. 
\end{proof}


\begin{figure}
\begin{center}
\includegraphics[width=13cm]{local_rules_transition}
\end{center}   
\caption{The local rule applied at every special original edge $e$ ($e_d=-1$), to produce a relaxed $d$-GS angular orientation from a weak $d$-GS angular orientation (arcs with no weight indication have weight $1$, arcs not shown on their edge have weight $0$). The edge $e$ yields $4$ simply directed ``green edges" in the intermediate step.}
\label{fig:local_rules_transition}
\end{figure}

\begin{prop}\label{prop:necessity_weak_GS}
If a $d$-map $G$ admits a weak $d$-GS angular orientation, then $G$ is weakly $d$-adapted. 
\end{prop}
\begin{proof}
As in Proposition~\ref{prop:necessity_GS}, the first step is to check that $G$ must be non-separable, i.e., that $G^+$ has no 2-cycle of star edges. Assume there is such a cycle $C'$, with $s$ the star vertex on $C'$, and $f$ the inner face of $G$ corresponding to $s$. Since $C'$ is not a special quadrangle, Lemma~\ref{lem:weak_compatible} and Lemma~\ref{lem:transition} ensure that 
$C$ has length at least $d$. Hence, $s$ has at least $d-1$ incident edges in the exterior of $C'$. Since $s$ is also incident to two edges on $C'$, it has degree larger than $d$, in contradiction with the fact that $G$ is a $d$-map.  


We now prove that any chordless non-facial cycle in $G$ has length at least $d$, by the same argument as in the proof of Proposition~\ref{prop:necessity_GS}. 
Let $X$ be the set of non-facial \emph{chordless}  
cycles of $G$ of length smaller than $d$. 
Assume $X$ is not empty, and let $C_0$ be a minimal element of $X$ (i.e., there is no other $C_1\in X$ such that the interior of $C_1$ is included in the interior of $C_0$). Since $C_0$ has length smaller than $d$ and is chordless, by Lemma~\ref{lem:weak_compatible} and Lemma~\ref{lem:transition} it can not be the enclosing cycle of a star cycle. 
Hence, there exists a face $f$ of $G$ 
inside $C$ that shares at least one edge with $C$, but such that the edges on $C$ and along $f$ do not form a contiguous set on the contour of $f$. Since $G$
is non-separable, this set of edges is neither contiguous on $C$. 
Hence, we are in the situation shown in  Figure~\ref{fig:C0}, with $L_1+L_2+2=\mathrm{length}(C_0)<d$ and 
$\ell_1+\ell_2+2=\mathrm{deg}(f)\leq d$, so $(L_2+\ell_1+2)+(L_1+\ell_2+2)<2d$, thus at least one of the two cycles on the right-side of  Figure~\ref{fig:C0} has length smaller than $d$, yielding a contradiction to the minimality of $C_0$. By contradiction, we conclude that any chordless non-facial cycle has length at least $d$.

Now, consider a non-facial cycle $C$ of $G$ having at least one chord. 
It admits a decomposition (at chords) into chordless cycles, as shown in Figure~\ref{fig:decomp_cycle}. If $C$ has at least one vertex inside, then one
of these chordless components is non-facial, hence has length at least $d$. Note that the length of $C$ is at least the length of any of its components, hence the length of $C$ is at least $d$.  

In order to conclude that $G$ is weakly $d$-adapted, the last case to consider is a non-facial cycle $C$ with no vertex inside, and at least two edges inside (all edges inside are chords). In that case, the components of the decomposition of $C$ into chords are facial cycles. Consider a pair of adjacent components of $C$, and let $C''$ be the contour of the union of these two faces. The length of $C''$
is at least $d-1$ since $G$ admits a weak $d$-GS angular orientation.  
In addition, since $C$ is not equal to $C''$, and since we assume all faces of $G$ to have degree at least $3$, the length of $C$ is larger than the length of $C''$, hence is at least~$d$. 
\end{proof}

\begin{figure}
\begin{center}
\includegraphics[width=13cm]{chord}
\end{center}   
\caption{Decomposition of a cycle into chordless components.}
\label{fig:decomp_cycle}
\end{figure}


%\end{document}
